Visual Semantic Parsing: From Images to Abstract Meaning Representation

The success of scene graphs for visual scene understanding has brought attention to the benefits of abstracting a visual input (e.g., image) into a structured representation, where entities (people and objects) are nodes connected by edges specifying their relations. Building these representations, however, requires expensive manual annotation in the form of images paired with their scene graphs or frames. These formalisms remain limited in the nature of entities and relations they can capture. In this paper, we propose to leverage a widely-used meaning representation in the field of natural language processing, the Abstract Meaning Representation (AMR), to address these shortcomings. Compared to scene graphs, which largely emphasize spatial relationships, our visual AMR graphs are more linguistically informed, with a focus on higher-level semantic concepts extrapolated from visual input. Moreover, they allow us to generate meta-AMR graphs to unify information contained in multiple image descriptions under one representation. Through extensive experimentation and analysis, we demonstrate that we can re-purpose an existing text-to-AMR parser to parse images into AMRs. Our findings point to important future research directions for improved scene understanding.

==> intro-v0.tex <==

%% There is debate on what it means to understand an image: briefly mention each of the relevant topics of captioning, SGG, and Situation Recognition (ignore object detection, etc.). Then talk about our proposal. The rest can go to Related Work.

%//NOTE: {\bf the intro. sounds more like a computer vision paper, and it takes a while to get to the linguisticy part. I am aware of this, and will need to address it later. For now, I want to make sure we tell a coherent story. And then may be we can change the order of events in the story. Need to shorten and make this more focused. Perhaps move some of these to related work.}

The ability to understand and describe a scene is fundamental for the development of truly intelligent systems, including autonomous vehicles, robots navigating an environment, or even simpler applications such as voice-based image retrieval. The early days of computer vision has seen a lot of work focusing on specific aspects of scene understanding, including object detection \cite{}, activity recognition \cite{}, human--object interaction \cite{}, and relation detection \cite{}, to name a few. More recently, scene graphs encoding the detected objects and their relationships are widely adopted as a semantic formalism for representing the content of an image \cite{johnson.etal.2015}.
Generating scene graphs from an image requires expensive and detailed annotations. As such,
others have attempted to understand an image by learning to describe it using language, a research area known as image captioning \cite{}.
%survey paper on image captioning, e.g., https://arxiv.org/abs/2107.06912
%plus original non-DN-based and DN-based image captioning work

With the advent of deep learning, automatic scene graph generation and image captioning have seen a lot of progress in recent years. Even the most impressive captioning models with SoTA performance in terms of the common n-gram based metrics have a tendency of generating similar generic captions for similar images, ignoring the more specific and distinctive aspects \cite{lindh.etal.2018}. 
As for scene graphs, not only their generation requires expensive manual annotation in the form of detected objects and their relations, but also they are very skewed in terms of the entity and relation types that they encode \cite{zellers.etal.2018}. %Neural Motifs paper
For example, in the scene graphs of Visual Genome \cite{}, clothing and parts make up over one-third of entity instances, and the geometric and possessive relations together account for more than 90\% of all relation instances.

\citet{yatskar.etal.2016} propose situation recognition, or visual semantic role labelling, as a linguistically-motivated approach to image understanding. Given an image, they draw on FrameNet \cite{} to predict a situation, that is composed of a verb (encoding the main event or activity depicted in the image), and an instantiated frame specifying the participants and their semantic roles.
Situation recognition generalizes activity recognition and human--object interaction, focusing on recognizing a {\it single} main activity and detecting its {\it frame-specific} participants (see Figure~\ref{fig1}). 

Here, we pose two fundamental questions: (i) How can we generalize situation recognition from images to capture not only the main event but all aspects of ``who did what to whom'', in the same way semantic parsing generalizes semantic role labelling on sentences; and (ii) Whether and in what ways such visual semantic parsing would help downstream vision-and-language tasks?
%
%//TODO what is AMR and what aspect of meaning it encodes; why are they appropriate for image semantics representation?
To answer (i), we propose to adpat 
Abstract Meaning Representation (AMR) \cite{banarescu.etal.2013}, which is a widely-adopted formalism for semantic parsing of sentences (and documents), to the visual domain. AMRs are rooted, directed, acyclic graphs with labels on edges (relations) and leaves (concepts) taken from PropBank \cite{palmer.etal.2005}. Recently, a number of high-performing neural network models have been developed for parsing a sentence into an AMR graph \cite{bevilacqua.etal.2021,xia.etal.2021}.
Our goal is to devise a visual semantic parser that can learn to represent the semantics of an image using an AMR graph. Two key challenges that we need to address include: (i) adapting a text-to-AMR model to learning AMRs from images, and (ii) achieving this goal in the absence of ground-truth annotations of images with their corresponding AMR graphs. 
%Unlike in situation recognition and scene graph generation, we do not have access to images paired with their AMR graphs. We thus need to rely on indirect supervision. 

//TODO provide a single image with its corresponding situation (frame), captions, SG, and the meta-AMR graph.

//TODO here refer to the SG vs. AMR analysis table.
\todo{Kalliopi and Afsaneh}

To answer (ii), ...
Representing the semantics of an image with AMRs provides many opportunities for improved down-stream tasks, including personalized captioning \cite{}, controlled captioning \cite{shizhe-chen.etal.2020,long-chen.etal.2021}, or group captioning \cite{li.etal.2020}. //TODO add how AMRs can be of use here

//TODO expand on these (e.g., visual storytelling? visual question answering? multimodal augmentation? explainability and compositional generalization?)

//TODO summary of contributions

% DNN-based image captioning: image-to-sequence problem
% image captioning can be: perceptual (focusing on low-level visual attributes), non-visual (reporting implicit or contextual information), or conceptual (visual entities and their relations).




==> relatedwork.tex <==

\paragraph{Applications of Abstract Meaning Representation (AMR).}

\todo{Not sure if we need a separate related work section.}

AMRs have been used for a variety of down-stream applications in natural language understanding, including abstractive and multi-document summarization \cite{liu.etal.2015,liao.etal.2018,hardy.vlachos.2018,naseem.etal.2021}, machine translation \cite{song.etal.2019}, and question answering \cite{kapanipathi.etal.2019}.

%Muti-document AMRs.
%\cite{liu.etal.2015,liao.etal.2018,naseem.etal.2021}

\paragraph{Image Understanding.}

Activity Recognition and Human--Object Interaction from images \cite{}.

Scene Graph Generation \cite{zhu.etal.2022.survey};
Image Captioning \cite{stefanini.etal.2021.survey};
Situation Recognition \cite{}.
